DecoSurf: Recursive Geodesic Patterns on Triangle Meshes

In this paper, we show that many complex patterns, which characterize the decorative style of many artisanal objects, can be generated by the recursive application of only four operators. Each operator is derived from tracing the isolines or the integral curves of geodesics fields generated from selected seeds on the surface. Based on this formulation, we present an interactive application that lets designers model complex recursive patterns directly on the object surface, without relying on parametrization. We support interaction on commodity hardware on meshes of a few million triangles, by combining light data structures together with an efficient approximate graph-based geodesic solver. We validate our approach by matching decoration styles from real-world photos, by analyzing the speed and accuracy of our geodesic solver, and by validating the interface with a user study.

==> 00_setup.tex <==
% !TEX root = ./scenegit.tex

% \usepackage{tikz}
% \usepackage{verbatim}
% \usepackage{xcolor}
\usepackage{xspace}
% \usetikzlibrary{shapes,decorations.markings,shapes.geometric,positioning,arrows,fadings}
% \usepackage{colortbl}

%%%%% For sectioning:
\newcommand{\parasection} [1] {\textsf{\textbf{#1}.}}
\newcommand{\bs}[1] {\textbf{\textsf{#1}}}

%%%%% For comments:
\newcommand{\oldversion } [1] { }
\newcommand{\ignorethis } [1] { }
\newcommand{\note       } [1] {\textcolor{red}{\textbf{Note:} {\slshape #1}}}
\newcommand{\smallnote  } [1] {{\small \{#1\}}}
\newcommand{\bignote    } [1] {\begin{quote} \textbf{Note:\ }
                               \slshape #1 \end{quote}}
\newcommand{\urgent } [1] {\textcolor{red}{\textbf{Urgent:}{#1}}}
\newcommand{\issues } [1] {\textcolor{blue}{\textbf{Issue:}{#1}}}
\newcommand{\missing} [1] {\textcolor{green}{\textbf{Missing:}{#1}}}
\newcommand{\jon    } [1] {\textcolor{red}{\textbf{j:} {\slshape #1}}}
\newcommand{\fabio  } [1] {\textcolor{orange}{\textbf{f:} {\slshape #1}}}
\newcommand{\gab    } [1] {\textcolor{purple}{\textbf{g:} {\slshape #1}}}
\newcommand{\edo    } [1] {\textcolor{green}{\textbf{e:} {\slshape #1}}}
\newcommand{\giacomo} [1] {\textcolor{blue}{\textbf{g:} {\slshape #1}}}
\newcommand{\enrico } [1] {\textcolor{purple}{\textbf{e:} {\slshape #1}}}
\newcommand{\fixme  } [1] {\textcolor{red}{\textbf{#1}}}
\newcommand{\fillit } [1] {\textcolor{cyan}{\textbf{fil:} {\slshape #1}}}
\newcommand{\maybe  } [1] {\textcolor{gray}{\textbf{maybe:} {#1}}}


%%%%% For referencing things:
\newcommand{\chapnum    } [1] {\ref{#1}}
\newcommand{\appnum     } [1] {\ref{#1}}
\newcommand{\sectnum    } [1] {\ref{#1}}
\newcommand{\tblnum     } [1] {\ref{#1}}
\newcommand{\fignum     } [1] {\ref{#1}}
\newcommand{\algnum     } [1] {\ref{#1}}
%\newcommand{\eqnnum     } [1] {\mbox{(\ref{#1})}}
\newcommand{\eqnnum     } [1] {\ref{#1}}
\newcommand{\chap       } [1] {Chapter~\chapnum{#1}}
\newcommand{\chaps      } [1] {Chapters~\chapnum{#1}}
\newcommand{\app        } [1] {Appendix~\appnum{#1}}
\newcommand{\apps       } [1] {Appendices~\appnum{#1}}
\newcommand{\sect       } [1] {Sec.~\sectnum{#1}}
\newcommand{\sects      } [1] {Sections~\sectnum{#1}}
\newcommand{\tbl        } [1] {Tab.~\tblnum{#1}}
\newcommand{\tbls       } [1] {Tables~\tblnum{#1}}
\newcommand{\fig        } [1] {Fig.~\fignum{#1}}
%\newcommand{\figure     } [1] {Figure~\fignum{#1}}
\newcommand{\figs       } [1] {Figures~\fignum{#1}}
\newcommand{\alg 		} [1] {Alg.~\algnum{#1}}
\newcommand{\eqn        } [1] {Equation~\eqnnum{#1}}
\newcommand{\eqns       } [1] {Equations~\eqnnum{#1}}

%%%%% For conditionally referencing things
\newcommand{\cfignum}[2]{\IfRefUndefinedExpandable{#1}{#2}{\fignum{#1}}}


%%%%% Latin:
%% \newcommand{\etal       }     {\textit{et~al.}} old; not like ACM style
% \newcommand{\etal       }     {{et~al.}}
% \newcommand{\apriori    }     {\textit{a~priori}}
% \newcommand{\aposteriori}     {\textit{a~posteriori}}
% \newcommand{\perse      }     {\textit{per~se}}
% \newcommand{\cf         }     {\textit{cf.}}
% \newcommand{\eg         }     {{e.g.,}}
% \newcommand{\Eg         }     {{E.g.,}}
% \newcommand{\ie         }     {{i.e.,}}
% \newcommand{\Ie         }     {{I.e.,}}

%%%%% Math symbols:
\newcommand{\Identity   }     {\mat{I}}
\newcommand{\Zero       }     {\mathbf{0}}
\newcommand{\Reals      }     {{\textrm{I\kern-0.18em R}}}
\newcommand{\isdefined  }     {\mbox{\hspace{0.5ex}:=\hspace{0.5ex}}}
%\newcommand{\implies    }     {\Longrightarrow}
\newcommand{\texthalf   }     {\ensuremath{\textstyle\frac{1}{2}}}
\newcommand{\half       }     {\ensuremath{\frac{1}{2}}}
\newcommand{\third      }     {\ensuremath{\frac{1}{3}}}
\newcommand{\fourth      }    {\ensuremath{\frac{1}{4}}}

%%%%% Math modifiers:
%\renewcommand{\vec      } [1] {{\text{\boldmath $\mathbit{#1}$}}}
\renewcommand{\vec      } [1] {\mathbf{#1}}
\newcommand{\mat        } [1] {{\text{\boldmath $\mathbit{#1}$}}}
\newcommand{\Approx     } [1] {\widetilde{#1}}
\newcommand{\change     } [1] {\mbox{{\footnotesize $\Delta$} \kern-3pt}#1}

%%%%% Math functions:
\newcommand{\Order      } [1] {O(#1)}
\newcommand{\set        } [1] {{\lbrace #1 \rbrace}}
\newcommand{\floor      } [1] {{\lfloor #1 \rfloor}}
\newcommand{\ceil       } [1] {{\lceil  #1 \rceil }}
\newcommand{\inverse    } [1] {{#1}^{-1}}
\newcommand{\transpose  } [1] {{#1}^\mathrm{T}}
\newcommand{\invtransp  } [1] {{#1}^{-\mathrm{T}}}


%%%%% Math functions with small (fixed) and large (expandable) forms:
\newcommand{\abs        } [1] {{| #1 |}}
\newcommand{\Abs        } [1] {{\left| #1 \right|}}
\newcommand{\norm       } [1] {{\| #1 \|}}
\newcommand{\Norm       } [1] {{\left\| #1 \right\|}}
\newcommand{\pnorm      } [2] {\norm{#1}_{#2}}
\newcommand{\Pnorm      } [2] {\Norm{#1}_{#2}}
\newcommand{\inner      } [2] {{\langle {#1} \, | \, {#2} \rangle}}
\newcommand{\Inner      } [2] {{\left\langle \begin{array}{@{}c|c@{}}
                               \displaystyle {#1} & \displaystyle {#2}
                               \end{array} \right\rangle}}
\newcommand{\argmin     } [1] {{\underset{#1}{\operatorname{argmin}}}}


\newcommand{\manif		} {\mathcal M}
\newcommand{\mesh		} [1] {\ensuremath{\textit{M}^{#1}}}
\newcommand{\meshm		} [1] {\ensuremath{\textit{M\hspace{0.01in}}'^{#1}}}
%\newcommand{\ops		} [1] {\ensuremath{\textit{ops}_{#1}}}
%\newcommand{\graph		} [1] {\ensuremath{\textit{graph}_{#1}}}
\newcommand{\meshtopo   }     {\textcolor{red}{topology}}
\newcommand{\med        }     {\emph{mesh edit distance}}
%\newcommand{\VERT       }     {\textsc{vertex}}
%\newcommand{\FACE       }     {\textsc{face}}

\newcommand{\opc        } [2] {{\ensuremath{#1 \leftrightarrow #2}}}
\newcommand{\opctight   } [2] {{\ensuremath{#1\hspace{-2pt}\rightarrow{}\hspace{-2pt}#2}}}
%\newcommand{\opa        } [1] {{\ensuremath{\epsilon \rightarrow #1}}}
%\newcommand{\opd        } [1] {{\ensuremath{#1 \rightarrow \epsilon}}}
%\newcommand{\opn        }     {\ensuremath{\epsilon \rightarrow \epsilon}}

\newcommand{\extalg     }     {Iterative-Greedy}


%\newcommand{\figlbl     } [1] {{\textbf{\textsf{#1}}}}
\newcommand{\figlbl     } [1] {{{\textsf{#1}}}}


\newcommand{\addinsetbox}[3]{\makebox[0pt]{\hspace{-#1}\raisebox{#2}{\fbox{\includegraphics[width=#3]{figures/blank.png}}}}}
\newcommand{\vhtext}[2]{\begin{sideways}\parbox{#1}{\centering#2}\end{sideways}}
\newcommand{\vhtextr}[2]{\begin{turn}{270}\parbox{#1}{\centering#2}\end{turn}}

% a b c d e
% f g h i j
% k l m n o
\newcommand{\includemesh}[2]{\includegraphics[width=#1]{figures/#2}}

\newcommand{\includemesha}[2]{\includegraphics[width=#1,trim=   0px  720px 1536px   0px,clip=true]{figures/#2}}
\newcommand{\includemeshb}[2]{\includegraphics[width=#1,trim= 384px  720px 1152px   0px,clip=true]{figures/#2}}
\newcommand{\includemeshc}[2]{\includegraphics[width=#1,trim= 768px  720px  768px   0px,clip=true]{figures/#2}}
\newcommand{\includemeshd}[2]{\includegraphics[width=#1,trim=1152px  720px  384px   0px,clip=true]{figures/#2}}
\newcommand{\includemeshe}[2]{\includegraphics[width=#1,trim=1536px  720px    0px   0px,clip=true]{figures/#2}}
\newcommand{\includemeshf}[2]{\includegraphics[width=#1,trim=   0px  360px 1536px 360px,clip=true]{figures/#2}}
\newcommand{\includemeshg}[2]{\includegraphics[width=#1,trim= 384px  360px 1152px 360px,clip=true]{figures/#2}}
\newcommand{\includemeshh}[2]{\includegraphics[width=#1,trim= 768px  360px  768px 360px,clip=true]{figures/#2}}
\newcommand{\includemeshi}[2]{\includegraphics[width=#1,trim=1152px  360px  384px 360px,clip=true]{figures/#2}}
\newcommand{\includemeshj}[2]{\includegraphics[width=#1,trim=1536px  360px    0px 360px,clip=true]{figures/#2}}
\newcommand{\includemeshk}[2]{\includegraphics[width=#1,trim=   0px    0px 1536px 720px,clip=true]{figures/#2}}
\newcommand{\includemeshl}[2]{\includegraphics[width=#1,trim= 384px    0px 1152px 720px,clip=true]{figures/#2}}
\newcommand{\includemeshm}[2]{\includegraphics[width=#1,trim= 768px    0px  768px 720px,clip=true]{figures/#2}}
\newcommand{\includemeshn}[2]{\includegraphics[width=#1,trim=1152px    0px  384px 720px,clip=true]{figures/#2}}
\newcommand{\includemesho}[2]{\includegraphics[width=#1,trim=1536px    0px    0px 720px,clip=true]{figures/#2}}

\newcommand{\includemeshat}[6]{\includegraphics[width=#1,trim=   0px+#2  720px+#3 1536px+#4   0px+#5,clip=true]{figures/#6}}
\newcommand{\includemeshbt}[6]{\includegraphics[width=#1,trim= 384px+#2  720px+#3 1152px+#4   0px+#5,clip=true]{figures/#6}}
\newcommand{\includemeshct}[6]{\includegraphics[width=#1,trim= 768px+#2  720px+#3  768px+#4   0px+#5,clip=true]{figures/#6}}
\newcommand{\includemeshdt}[6]{\includegraphics[width=#1,trim=1152px+#2  720px+#3  384px+#4   0px+#5,clip=true]{figures/#6}}
\newcommand{\includemeshet}[6]{\includegraphics[width=#1,trim=1536px+#2  720px+#3    0px+#4   0px+#5,clip=true]{figures/#6}}
\newcommand{\includemeshft}[6]{\includegraphics[width=#1,trim=   0px+#2  360px+#3 1536px+#4 360px+#5,clip=true]{figures/#6}}
\newcommand{\includemeshgt}[6]{\includegraphics[width=#1,trim= 384px+#2  360px+#3 1152px+#4 360px+#5,clip=true]{figures/#6}}
\newcommand{\includemeshht}[6]{\includegraphics[width=#1,trim= 768px+#2  360px+#3  768px+#4 360px+#5,clip=true]{figures/#6}}
\newcommand{\includemeshit}[6]{\includegraphics[width=#1,trim=1152px+#2  360px+#3  384px+#4 360px+#5,clip=true]{figures/#6}}
\newcommand{\includemeshjt}[6]{\includegraphics[width=#1,trim=1536px+#2  360px+#3    0px+#4 360px+#5,clip=true]{figures/#6}}
\newcommand{\includemeshkt}[6]{\includegraphics[width=#1,trim=   0px+#2    0px+#3 1536px+#4 720px+#5,clip=true]{figures/#6}}
\newcommand{\includemeshlt}[6]{\includegraphics[width=#1,trim= 384px+#2    0px+#3 1152px+#4 720px+#5,clip=true]{figures/#6}}
\newcommand{\includemeshmt}[6]{\includegraphics[width=#1,trim= 768px+#2    0px+#3  768px+#4 720px+#5,clip=true]{figures/#6}}
\newcommand{\includemeshnt}[6]{\includegraphics[width=#1,trim=1152px+#2    0px+#3  384px+#4 720px+#5,clip=true]{figures/#6}}
\newcommand{\includemeshot}[6]{\includegraphics[width=#1,trim=1536px+#2    0px+#3    0px+#4 720px+#5,clip=true]{figures/#6}}

%%%%%% PAPER %%%%%%%%

\newcommand{\AppName}{\emph{SceneGit}\xspace}


\renewcommand{\topfraction}{0.9}    % max fraction of floats at top
\setcounter{topnumber}{2}
\setcounter{totalnumber}{4}     % 2 may work better
\renewcommand{\textfraction}{0.07}  % allow minimal text w. figs
\renewcommand{\floatpagefraction}{0.7}  % require fuller float pages
\renewcommand{\dblfloatpagefraction}{0.7}   % require fuller float pages
\renewcommand{\thefootnote}{\fnsymbol{footnote}}

\DeclareMathOperator*{\avg}{avg}
\DeclareMathOperator*{\area}{area}
\DeclareMathOperator*{\mindist}{min-dist}

\newcommand{\quarterpagewidth}{0.8in} %1.0
\newcommand{\thirdpagewidth  }{1.8in} %2.0
\newcommand{\halfpagewidth   }{2.8in} %3.0
\newcommand{\fullpagewidth   }{5.8in} %6.0


